Most Classic Problems Remain NP-hard on Relative Neighborhood Graphs and their Relatives

Proximity graphs have been studied for several decades, motivated by applications in computational geometry, geography, data mining, and many other fields. However, the computational complexity of classic graph problems on proximity graphs mostly remained open. We now study 3-Colorability, Dominating Set, Feedback Vertex Set, Hamiltonian Cycle, and Independent Set on the proximity graph classes relative neighborhood graphs, Gabriel graphs, and relatively closest graphs. We prove that all of the problems remain NP-hard on these graphs, except for 3-Colorability and Hamiltonian Cycle on relatively closest graphs, where the former is trivial and the latter is left open. Moreover, for every NP-hard case we additionally show that no $2^{o(n^{1/4})}$-time algorithm exists unless the ETH fails, where n denotes the number of vertices.

==> figs/tikzpreamble.tex <==
\RequirePackage{xargs}     

\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{math}
\usetikzlibrary{calc}

\newcommand{\tikzpreamble}{\def\teps{0.075}
	\def\nsc{0.33}
	\def\tanS{1.7320508}
	\def\bsc{0.075}
	\tikzstyle{xnode}=[circle,scale=\nsc,draw,fill=white];
	\tikzstyle{xnodeA}=[circle,scale=\nsc,fill=white,draw=red];
	\tikzstyle{xnodeB}=[circle,scale=\nsc,fill=lightgray,draw=green];
	\tikzstyle{xnodeC}=[circle,scale=\nsc,fill=black,draw=blue];
	\tikzstyle{xnodex}=[circle,fill,scale=\nsc,draw];
	\tikzstyle{xnodey}=[diamond,fill,scale=\nsc,draw];
	\tikzstyle{xedge}=[thick,-];
	\tikzstyle{xedgex}=[thick,-,dashed];
	\tikzstyle{xedgedot}=[thick,-,dotted];
	
	\tikzstyle{xpath}=[color=blue,opacity=0.25,line cap=round,line width=6pt];
	\tikzstyle{xpathS}=[color=blue!40!white,opacity=0.3,line cap=round,line join=round,line width=5pt];
	\tikzstyle{xpathSx}=[color=green!40!black,opacity=0.3,line cap=round,line join=round,line width=5pt];
	\tikzstyle{xpathx}=[color=magenta,opacity=0.40,line cap=round,line width=6pt];
	\tikzstyle{xpathy}=[color=green,opacity=0.40,line cap=round,line width=6pt];
	
	\tikzstyle{xhili}=[circle,scale=1.25,opacity=0.25,fill,color=orange,draw];
	\tikzstyle{xhiliS}=[circle,scale=0.75,opacity=0.25,fill,color=orange,draw];
	\tikzstyle{xhiliIS}=[circle,scale=1.25,opacity=0.25,fill,color=magenta,draw];
	\tikzstyle{xxhili}=[scale=1.25,opacity=0.25,fill,color=cyan,draw];
}

\newcommand{\theexgraph}{\node (v1) at (0,0)[xnode,label=-90:{$v_1$}]{};
	\node (v2) at (1*\xr,0)[xnode,label=-90:{$v_2$}]{};
	\node (v3) at (2*\xr,0)[xnode,label=-90:{$v_3$}]{};
	\node (v4) at (3*\xr,0)[xnode,label=-90:{$v_4$}]{};
	\draw[xedge] (v1) to [out=45,in=135]node[midway,below]{$e_1$}(v2);
	\draw[xedge] (v1) to [out=90,in=90]node[midway,below]{$e_2$}(v4);
	\draw[xedge] (v2) to [out=45,in=135]node[midway,below]{$e_3$}(v3);
	\draw[xedge] (v2) to [out=60,in=120]node[midway,below]{$e_4$}(v4);
}

\newcommand{\Grid}[9]{
	\foreach\x in {0,...,#2}{
		\foreach \y in {0,...,#3}{
			\node (#1\x\y) at (#8*\x*\xr+#4*\xr,#9*\y*\yr+#5*\yr)[xnode,#6]{};
		}
	}
	\ifnum#3>0
	\pgfmathsetmacro\yx{int(#3 - 1)}
	\foreach \x in {0,...,#2}
	\foreach \y [count=\yi] in {0,...,\yx}  
	\draw[#7] (#1\x\y)--(#1\x\yi) ;
	\fi
	\ifnum#2>0
	\pgfmathsetmacro\yx{int(#2 - 1)}
	\foreach \x in {0,...,#3}
	\foreach \y [count=\yi] in {0,...,\yx}  
	\draw[#7] (#1\y\x)--(#1\yi\x) ;
	\fi
}



\newcommand{\bufferhelp}[5]{
	\node (#1!#2Cb) at (+#3*\xr,+#4*\yr-1*\teps*\xr)[xnode,scale=#5]{};
	\node (#1!#2Cl) at (+#3*\xr-1*\teps*\xr,+#4*\yr+0*\teps*\xr)[xnode,scale=#5]{};
	\node (#1!#2Cr) at (+#3*\xr+1*\teps*\xr,+#4*\yr+0*\teps*\xr)[xnode,scale=#5]{};
	\node (#1!#2Ct) at (+#3*\xr,+#4*\yr+1*\teps*\xr)[xnode,scale=#5]{};
	\foreach\x/\y in {b/l,l/t,t/r,r/b}{\draw[-] (#1!#2C\x) to (#1!#2C\y);}
}
\newcommand{\buffer}[4]{
	\begin{scope}[shift={(#2*\xr cm,#3*\yr cm)}]
		\fill[white] (-4*\teps*\xr,-4*\teps*\yr) rectangle (4*\teps*\xr,4*\teps*\yr);
		\node (#1!tl) at (-1*\xr*\teps,+1*\teps*\yr)[xnode,scale=#4]{};
		\node (#1!tr) at (+1*\xr*\teps,+1*\teps*\yr)[xnode,scale=#4]{};
		\node (#1!br) at (+1*\xr*\teps,-1*\teps*\yr)[xnode,scale=#4]{};
		\node (#1!bl) at (-1*\xr*\teps,-1*\teps*\yr)[xnode,scale=#4]{};
		
		\bufferhelp{#1}{t}{0}{3*\teps}{#4}
		\bufferhelp{#1}{r}{3*\teps}{0}{#4}
		\bufferhelp{#1}{b}{0}{-3*\teps}{#4}
		\bufferhelp{#1}{l}{-3*\teps}{0}{#4}
		
		\foreach\x/\y in {tl/tCb,tl/lCr,tr/tCb,tr/rCl,bl/bCt,bl/lCr,br/bCt,br/rCl}{\draw[-] (#1!\x) to (#1!\y);}
	\end{scope}
}


\newcommandx{\hbuffer}[6][6=]{
	\begin{scope}[shift={(#2*\xr cm,#3*\yr cm)},rotate=#5]
		\fill[white] (-3*\xr*\teps-\xr*\teps/\tanS,0) rectangle (3*\xr*\teps-\xr*\teps/\tanS,4*\teps*\yr);
		\foreach\x in{0,1,2,3,4}{\node (#1!b\x) at (\x*\xr*\teps-2*\xr*\teps,0*\teps*\yr)[xnode,scale=#4]{};
			\ifnum\x>0
			\pgfmathsetmacro{\xx}{\x-1};
			\draw[-] (#1!b\xx) to (#1!b\x);
			\fi
		}
		
		\node (#1!tl) at (-1*\xr*\teps,+1*\teps*\yr)[xnode,scale=#4]{};
		\node (#1!tr) at (+1*\xr*\teps,+1*\teps*\yr)[xnode,scale=#4]{};
		
		\bufferhelp{#1}{t}{0}{3*\teps}{#4}
		
		\node (#1!lTl) at (-3*\xr*\teps-\xr*\teps/\tanS,0)[xnode,scale=#4]{};
		\node (#1!lTt) at (-3*\xr*\teps,1*\teps*\yr)[xnode,scale=#4]{};
		\node (#1!lTr) at (-3*\xr*\teps+\xr*\teps/\tanS,0)[xnode,scale=#4]{};
		\draw[-,#6] (#1!lTl) to (#1!lTt) to (#1!lTr) to (#1!lTl);
		
		\node (#1!rTl) at (+3*\xr*\teps-\xr*\teps/\tanS,0)[xnode,scale=#4]{};
		\node (#1!rTt) at (+3*\xr*\teps,1*\teps*\yr)[xnode,scale=#4]{};
		\node (#1!rTr) at (+3*\xr*\teps+\xr*\teps/\tanS,0)[xnode,scale=#4]{};
		\draw[-,#6] (#1!rTl) to (#1!rTt) to (#1!rTr) to (#1!rTl);
		
		\foreach\x/\y in {tl/tCb,tr/tCb,tl/b1,tr/b3,lTr/b0,rTl/b4}{\draw[-] (#1!\x) to (#1!\y);}
		
	\end{scope}
}


\newcommand{\fourzerogadget}{
	\foreach \a/\b in {-3/3,-3/2,-3/1,-3/0,-2/0,-1/3,-1/2,-1/1,-1/0,0/0,1/3,1/2,1/1,1/0,
		-1/-1,-1/-2,0/-2,1/-2,2/-2,3/-2,3/-1,3/0,3/1,3/2,3/3} {\node (P\a!\b) at(\a*\xr,\b*\yr) [xnode,color=blue]{} ;}
	\foreach \b in {-3,...,3} {\buffer{B-4!\b}{-4}{\b}{\bsc}}
	\foreach \b in {-3,-2,-1} {\buffer{B-3!\b}{-3}{\b}{\bsc}}
	\foreach \b in {-3,-2,-1,1,2,3} {\buffer{B-2!\b}{-2}{\b}{\bsc}}
	\buffer{B-1!-3}{-1}{-3}{\bsc}
	\foreach \b in {-3,-1,1,2,3} {\buffer{B0!\b}{0}{\b}{\bsc}}
	\foreach \b in {-3,-1} {\buffer{B1!\b}{1}{\b}{\bsc}}
	\foreach \b in {-3,-1,0,1,2,3} {\buffer{B2!\b}{2}{\b}{\bsc}}
	\buffer{B3!-3}{3}{-3}{\bsc}
	\foreach \b in {-3,...,3} {\buffer{B4!\b}{4}{\b}{\bsc}}
	\foreach \a/\b in {-4/-3,-4/-2,-4/-1,-4/0,-4/1,-4/2,
		-3/-3,-3/-2,
		-2/-3,-2/-2,-2/1,-2/2,
		0/1,0/2,
		2/-1,2/0,2/1,2/2,
		4/-3,4/-2,4/-1,4/0,4/1,4/2} {
		\pgfmathsetmacro{\p}{int(\b+1)};
		\draw [-] (B\a!\b!tCt) -- (B\a!\p!bCb);
	}
	\foreach \a/\b in {-3/-1,-2/-1,-1/-3,0/-3,0/-1,1/-3,1/-1,2/-3,3/-3} {
		\pgfmathsetmacro{\p}{int(\b+1)};
		\draw [-] (B\a!\b!tCt) -- (P\a!\p);
	}
	\foreach \a/\b in {-2/0,0/-2,0/0,1/-2,2/-2} {
		\pgfmathsetmacro{\p}{int(\b+1)};
		\draw [-] (P\a!\b) -- (B\a!\p!bCb);
	}
	\foreach \a/\b in {-3/0,-3/1,-3/2,-1/-2,-1/-1,-1/0,-1/1,-1/2,1/0,1/1,1/2,
		3/-2,3/-1,3/0,3/1,3/2} {
		\pgfmathsetmacro{\p}{int(\b+1)};
		\draw [-] (P\a!\b) -- (P\a!\p);
	}
	\foreach \a/\b in {-4/-3,-3/-3,-2/-3,-1/-3,0/-3,1/-3,2/-3,3/-3,
		-4/-2,-3/-2,
		-4/-1,-3/-1,0/-1,1/-1} {
		\pgfmathsetmacro{\p}{int(\a+1)};
		\draw [-] (B\a!\b!rCr) -- (B\p!\b!lCl);
	}
	\foreach \a/\b in {-2/-2,-2/-1,2/-1,-4/0,2/0,-4/1,-2/1,0/1,2/1,-4/2,-2/2,0/2,2/2,
		-4/3,-2/3,0/3,2/3} {
		\pgfmathsetmacro{\p}{int(\a+1)};
		\draw [-] (B\a!\b!rCr) -- (P\p!\b);
	}
	\foreach \a/\b in {3/-2,-1/-1,3/-1,1/0,3/0,-3/1,-1/1,1/1,3/1,-3/2,-1/2,1/2,3/2,
		-3/3,-1/3,1/3,3/3} {
		\pgfmathsetmacro{\p}{int(\a+1)};
		\draw [-] (P\a!\b) -- (B\p!\b!lCl);
	}
	\foreach \a/\b in {-1/-2,0/-2,1/-2,2/-2,-3/0,-2/0,-1/0,0/0} {
		\pgfmathsetmacro{\p}{int(\a+1)};
		\draw [-] (P\a!\b) -- (P\p!\b);
	}
	\foreach \a in {-4,...,4} {
		\foreach \b in {-3,...,2} {\node at (\a*\xr,\b*\yr+0.5*\yr) [xnode,scale=0.5]{};}
	}
	\foreach \a in {-4,...,3} {
		\foreach \b in {-3,...,3} {\node at (\a*\xr + 0.5*\xr,\b*\yr) [xnode,scale=0.5] {};}
	}
}

\newcommand{\threeonegadget}{
	\foreach \a/\b in {-3/3,-3/2,-3/1,-3/0,-2/0,-1/0,0/3,0/2,0/1,0/0,0/-1,0/-2,0/-3,1/0,2/0,
		3/3,3/2,3/1,3/0}
	{\node (P\a!\b) at(\a*\xr,\b*\yr) [xnode,color=blue]{} ;}
	\foreach \b in {-3,...,3} {\buffer{B-4!\b}{-4}{\b}{\bsc}}
	\foreach \b in {-3,-2,-1} {\buffer{B-3!\b}{-3}{\b}{\bsc}}
	\foreach \b in {-3,-2,-1,1,2,3} {\buffer{B-2!\b}{-2}{\b}{\bsc}}
	\foreach \b in {-3,-2,-1,1,2,3} {\buffer{B-1!\b}{-1}{\b}{\bsc}}
	\foreach \b in {-3,-2,-1,1,2,3} {\buffer{B1!\b}{1}{\b}{\bsc}}
	\foreach \b in {-3,-2,-1,1,2,3} {\buffer{B2!\b}{2}{\b}{\bsc}}
	\foreach \b in {-3,-2,-1} {\buffer{B3!\b}{3}{\b}{\bsc}}
	\foreach \b in {-3,...,3} {\buffer{B4!\b}{4}{\b}{\bsc}}
	\foreach \a/\b in {-4/-3,-4/-2,-4/-1,-4/0,-4/1,-4/2,
		-3/-3,-3/-2,
		-2/-3,-2/-2,-2/1,-2/2,
		-1/-3,-1/-2,-1/1,-1/2,
		1/-3,1/-2,1/1,1/2,
		2/-3,2/-2,2/1,2/2,
		3/-3,3/-2,
		4/-3,4/-2,4/-1,4/0,4/1,4/2} {
		\pgfmathsetmacro{\p}{int(\b+1)};
		\draw [-] (B\a!\b!tCt) -- (B\a!\p!bCb);
	}
	\foreach \a/\b in {-3/-1,-2/-1,-1/-1,1/-1,2/-1,3/-1} {
		\pgfmathsetmacro{\p}{int(\b+1)};
		\draw [-] (B\a!\b!tCt) -- (P\a!\p);
	}
	\foreach \a/\b in {-2/0,-1/0,1/0,2/0} {
		\pgfmathsetmacro{\p}{int(\b+1)};
		\draw [-] (P\a!\b) -- (B\a!\p!bCb);
	}
	\foreach \a/\b in {-3/0,-3/1,-3/2,0/-3,0/-2,0/-1,0/0,0/1,0/2,
		3/0,3/1,3/2} {
		\pgfmathsetmacro{\p}{int(\b+1)};
		\draw [-] (P\a!\b) -- (P\a!\p);
	}
	\foreach \a/\b in {-4/-3,-3/-3,-2/-3,1/-3,2/-3,3/-3,
		-4/-2,-3/-2,-2/-2,1/-2,2/-2,3/-2,
		-4/-1,-3/-1,-2/-1,1/-1,2/-1,3/-1,
		-2/1,1/1,-2/2,1/2,-2/3,1/3} {
		\pgfmathsetmacro{\p}{int(\a+1)};
		\draw [-] (B\a!\b!rCr) -- (B\p!\b!lCl);
	}
	\foreach \a/\b in 	{-1/-3,-1/-2,-1/-1,-4/0,-4/1,-1/1,2/1,
		-4/2,-1/2,2/2,-4/3,-1/3,2/3} {
		\pgfmathsetmacro{\p}{int(\a+1)};
		\draw [-] (B\a!\b!rCr) -- (P\p!\b);
	}
	
	\foreach \a/\b in 	{0/-3,0/-2,0/-1,3/0,-3/1,0/1,3/1,
		-3/2,0/2,3/2,-3/3,0/3,3/3} {
		\pgfmathsetmacro{\p}{int(\a+1)};
		\draw [-] (P\a!\b) -- (B\p!\b!lCl);
	}
	\foreach \a/\b in {-3/0,-2/0,-1/0,0/0,1/0,2/0} {
		\pgfmathsetmacro{\p}{int(\a+1)};
		\draw [-] (P\a!\b) -- (P\p!\b);
	}
	\foreach \a in {-4,...,4} {
		\foreach \b in {-3,...,2} {\node at (\a*\xr,\b*\yr+0.5*\yr) [xnode,scale=0.5]{};}
	}
	\foreach \a in {-4,...,3} {
		\foreach \b in {-3,...,3} {\node at (\a*\xr + 0.5*\xr,\b*\yr) [xnode,scale=0.5] {};}
	}
}

\newcommand{\twotwogadget}{
	\foreach \a/\b in 	{-3/3,-3/2,-3/1,-3/0,-2/0,-1/0,0/0,0/1,0/2,0/3,
		0/-1,0/-3,0/-2,
		1/0,2/0,3/0,3/-1,3/-2,3/-3}
	{\node (P\a!\b) at(\a*\xr,\b*\yr) [xnode,color=blue]{} ;}
	\foreach \b in {-3,...,3} {\buffer{B-4!\b}{-4}{\b}{\bsc}}
	\foreach \b in {-3,...,3} {\buffer{B4!\b}{4}{\b}{\bsc}}
	\foreach \a/\b in {-3/-1,-2/3,-2/2,-2/1,-2/-1,-2/-3,-1/3,-1/2,
		-1/1,-1/-1,-1/-3,1/3,1/1,1/-1,1/-2,
		1/-3,2/3,2/1,2/-1,2/-2,2/-3,3/1,1/2,2/2,3/2,3/3,
		-1/-2,-2/-2,-3/-2,-3/-3}
	{\buffer{B\a!\b}{\a}{\b}{\bsc}}
	
	\foreach \a/\b in {-4/-3,-4/-2,-4/-1,-4/0,-4/1,-4/2,
		-3/-3,-3/-2,
		-2/1,-2/2,-2/-3,-2/-2,
		-1/1,-1/2,-1/-3,-1/-2,
		1/-3,1/-2,1/1,1/2,
		2/-3,2/-2,2/1,2/2,
		3/1,3/2,
		4/-3,4/-2,4/-1,4/0,4/1,4/2} {
		\pgfmathsetmacro{\p}{int(\b+1)};
		\draw [-] (B\a!\b!tCt) -- (B\a!\p!bCb);
	}
	
	\foreach \a/\b in {-3/-1,-2/-1,-1/-1,
		1/-1,2/-1} {
		\pgfmathsetmacro{\p}{int(\b+1)};
		\draw [-] (B\a!\b!tCt) -- (P\a!\p);
	}
	vertical vertex to buffer
	\foreach \a/\b in {-2/0,-1/0,1/0,2/0,3/0} {
		\pgfmathsetmacro{\p}{int(\b+1)};
		\draw [-] (P\a!\b) -- (B\a!\p!bCb);
	}
	\foreach \a/\b in {-3/2,-3/1,-3/0,0/-3,0/-2,0/-1,0/0,0/1,0/2,
		3/-3,3/-2,3/-1} {
		\pgfmathsetmacro{\p}{int(\b+1)};
		\draw [-] (P\a!\b) -- (P\a!\p);
	}
	\foreach \a/\b in {-4/-3,-3/-3,-2/-3,1/-3,
		-4/-2,-3/-2,-2/-2,1/-2,
		-4/-1,-3/-1,-2/-1,1/-1,
		-2/1,1/1,2/1,3/1,
		-2/2,1/2,2/2,3/2,
		-2/3,1/3,2/3,3/3} {
		\pgfmathsetmacro{\p}{int(\a+1)};
		\draw [-] (B\a!\b!rCr) -- (B\p!\b!lCl);
	}
	\foreach \a/\b in {-4/3,-1/3,-4/2,-1/2,-4/1,-1/1,-4/0,
		-1/-1,2/-1,-1/-2,2/-2,-1/-3,2/-3} {
		\pgfmathsetmacro{\p}{int(\a+1)};
		\draw [-] (B\a!\b!rCr) -- (P\p!\b);
	}
	\foreach \a/\b in {-3/3,0/3,-3/2,0/2,-3/1,0/1,
		0/-1,3/-1,0/-2,3/-2,0/-3,3/-3} {
		\pgfmathsetmacro{\p}{int(\a+1)};
		\draw [-] (P\a!\b) -- (B\p!\b!lCl);
	}
	\foreach \a/\b in {-3/0,-2/0,-1/0,0/0,1/0,2/0} {
		\pgfmathsetmacro{\p}{int(\a+1)};
		\draw [-] (P\a!\b) -- (P\p!\b);
	}
	\foreach \a in {-4,...,4} {
		\foreach \b in {-3,...,2} {\node at (\a*\xr,\b*\yr+0.5*\yr) [xnode,scale=0.5]{};}
	}
	\foreach \a in {-4,...,3} {
		\foreach \b in {-3,...,3} {\node at (\a*\xr + 0.5*\xr,\b*\yr) [xnode,scale=0.5] {};}
	}
}




